Learning Robust Hybrid Control Barrier Functions for Uncertain Systems

The need for robust control laws is especially important in safety-critical applications. We propose robust hybrid control barrier functions as a means to synthesize control laws that ensure robust safety. Based on this notion, we formulate an optimization problem for learning robust hybrid control barrier functions from data. We identify sufficient conditions on the data such that feasibility of the optimization problem ensures correctness of the learned robust hybrid control barrier functions. Our techniques allow us to safely expand the region of attraction of a compass gait walker that is subject to model uncertainty.

==> chapter/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented a framework for learning safe control laws for hybrid systems. We introduced HCBFs and sufficient conditions under which an HCBF based control law guarantees safety, i.e., a desired safe set is made forward invariant. We then showed how to learn such HCBFs from data using an optimization-based framework. We gave sufficient conditions under which feasible solutions to the optimization problem are valid HCBFs, and illustrated our methods on two case studies.  %, including a compass gait walker.  
Future work will look to extend this approach to hybrid systems described by differential \emph{inclusions}, so as to be applicable to systems with friction and stiction, as well as to develop statistical guarantees of correctness to alleviate the sampling burden of our method.
